Lung Function Measurement with Multiple-Breath-Helium Washout System

Multiple-breath-washout (MBW) measurements are regarded as a sensitive technique which can reflect the ventilation inhomogeneity of respiratory airways. Typically nitrogen is used as the tracer gas and is washed out by pure oxygen in multi-breath-nitrogen (MBNW) washout tests. In this work, instead of using nitrogen, helium is used as the tracer gas and a multiple-helium-breath-washout (MBHW) system has been developed for the lung function study. A commercial quartz tuning fork with a resonance frequency of 32768 Hz has been used for detecting the change of the respiratory gas density. The resonance frequency of the tuning fork decreases linearly with increasing density of the surrounding gas. Knowing the CO2 concentration from the infrared carbon dioxide detector, the helium concentration can be determined. Results from 12 volunteers (3 mild asthmatics, 2 smokers, 1 with asthma history, 1 with COPD history, 5 normal) have shown that mild asthmatics have higher ventilation inhomogeneity in either conducting or acinar airways (or both). A feature has been found in single breath washout curve from 4 smokers with different length of smoking history which may indicate the early stage of respiratory ventilation inhomogeneity.

==> MEP2011bib.tex <==
@STRING(PRL="Phys. Rev. Lett.")
@STRING(RMP="Rev. Mod. Phys.")
@STRING(APL="Appl. Phys. Lett.")
@STRING(PRB="Phys. Rev. B")
@STRING(ASS="Appl. Surf. Sci.")
@STRING(PE="Physica E")
@STRING(RSI="Rev. Sci. Instrum.")
@STRING(NANO="Nanotechnology")
@STRING(JAP="J. Appl. Phys")
@STRING(JPI="J. Appl. Physiol")

%%%intro%%%%%%%%%%%%%%
@BOOK{Engel_book,
  AUTHOR="Engel, L. A. and Paiva, M.",
  TITLE="Gas mixing and distribution in the lung (Lung biology in health and disease) : Chapter 7",
  PUBLISHER = "Marcel Dekker, New York" ,
  EDITION = "1st",
  PAGES = "296",
  YEAR = 1985,
}

@ARTICLE{Sylvia2005,
   AUTHOR="Muylem, A. V. and Verbanck, S. and Estenne, M.",
   TITLE="{Monitoring the lung periphery of transplanted lungs}",
   JOURNAL="Repiratory Physiology and Neurobiology",
   VOLUME="148",
   PAGES="141-151",
   YEAR="2005"
} 

@ARTICLE{Bouhuys1956,
   AUTHOR="Bouhuys, A. and Hagstam, K. E. and Lundin, G.",
   TITLE="Efficiency of pulmonary ventilation during rest and light exercise.",
   JOURNAL="Acta. Physiol. Scand.",
   VOLUME="35",
   PAGES="289-304",
   YEAR="1956"
} 

@ARTICLE{Fowler1949,
   AUTHOR="Fowler, W. S.",
   TITLE="Lung function studies. III. Uneven Pulmonary Ventilation in Normal Subjects and in Patients with Pulmonary Disease",
   JOURNAL="J. Appl. Physiol.",
   VOLUME="2",
   PAGES="283-299",
   YEAR="1949"
} 

@ARTICLE{Paiva_Engel1984,
   AUTHOR="Paiva, M. and Engel, L. A.",
   TITLE="Model analysis of gas distribution within human acinus.",
   JOURNAL="J. Appl. Physiol.",
   VOLUME="56",
   PAGES="418-425",
   YEAR="1984"
}

@ARTICLE{Paiva_Engel1987,
   AUTHOR="Paiva, M. and Engel, L. A.",
   TITLE="Theoretical Studies of Gas Mixing and Ventilation Distribution in the Lung.",
   JOURNAL="Physiological Reviews",
   VOLUME="67",
   PAGES="751-797",
   YEAR="1987"
} 

@ARTICLE{Paiva1982,
   AUTHOR="Paiva, M. and Van Muylem, A. and Engel, L. A.",
   TITLE="The slope of phase III in multibreath nitrogen washout and washin.",
   JOURNAL="Bull. Eur. Physiopathol. Respir.",
   VOLUME="18",
   PAGES="273-280",
   YEAR="1982"
}

@ARTICLE{Paiva1984, 
   AUTHOR="Paiva, M. and Van Muylem, A. and Raves, P. and Yernault, J. C.",
   TITLE="Inspired volume dependence of the slope of the alveolar plateau", 
   JOURNAL="Respir. Physiol."
   VOLUME="56",
   YEAR="1984",
   PAGES="309-325"
}

@Article{Paiva1995,   %MBNW_gravity
author = {Prisk, G. K. and Guy, H. J. and Elliott, A. R. and Paiva, M. and West, J. B.},
title = {{Ventilatory inhomogeneity determined from multiple-breath washouts during sustained microgravity on Spacelab SLS-1}},
journal = {J. Appl. Physiol.},
volume = {78},
number = {2},
pages = {597-607},
year = {1995},
}

@ARTICLE{SylviaCOPD,
   AUTHOR="Verbanck, S. and Schuermans, D. and Van Muylem, A, and Melot, C. and Noppen, M. and Vincken, W. and Paiva, M.",
   TITLE="Conductive and acinar lung-zone contributions to ventialtion inhomogeneity in COPD.",
   JOURNAL="Am. J. Respir. Crit. Care Med.",
   VOLUME="157",
   PAGES="1573-1577",
   YEAR="1998"
}

@ARTICLE{PEF,
   AUTHOR="Nunn, A. J. and Gregg, I.",
   TITLE="New Regression Equations for Predicting Peak Expiratory Flow in Adults.",
   JOURNAL="BMJ",
   VOLUME="298",
   PAGES="1068-1070",
   NUMBER="1",
   YEAR="1989"
} 

@ARTICLE{Paiva1975,
   AUTHOR="Paiva, M.",
   TITLE="Two new pulmonary functional indexes suggested by a simple mathematical model.",
   JOURNAL="Respir. Physiol.",
   VOLUME="32",
   PAGES="389-403",
   YEAR="1975"
}

@Article{newth1997,
author = "Newth, C. J. and Enright, P. and Johnson, R. L.",
title = "Multiple-breath nitrogen washout techniques including measurements with patients on ventilators",
journal = "Eur. Respir. J.",
volume = "10",
number = "10",
pages = "2174-2185",
year = "1997"
}

@ARTICLE{Robertson1950,
   AUTHOR="Robertson, J. S. and Siri, W. E. and Jones, H. B.",
   TITLE="Lung ventilation patterns determined by analysis of nitrogen elimination rates; use of the mass spectrometer as a continuous gas analyzer.",
   JOURNAL="J. Clin. Invest.",
   VOLUME="29",
   PAGES="577-590",
   YEAR="1950"
} 

@ARTICLE{Sylvia2007,
   AUTHOR="Downie, S. R. and Salome, C. M. and Verbanck, S, and Thompson, B. and Berend, N. and King, G.",
   TITLE="Ventilation heterogeneity is a major determinant of airway hyperresponsiveness in asthma, independent of airway inflammation.",
   JOURNAL="Throax",
   VOLUME="62",
   PAGES="684-689",
   YEAR="2007"
}

@ARTICLE{Sylvia2004,
   AUTHOR="Downie, S. R. and Verbanck, S, and Gunnar, U. and King, G. and Salome, C. and Berend, N. ",
   TITLE="Detection of small and large airway heterogeneity in asthma by the multiple breath nitrogen washout test.",
   JOURNAL="Respirology",
   VOLUME="9S:2",
   PAGES="A31",
   YEAR="2004"
}

@ARTICLE{Aurora2005,
   AUTHOR="Aurora, P. and Bush, A. and Gustafsson, P. and Oliver, C. and Wallis, C. and Price, J. and Stroobant, J. and Carr, S. and Stocks, J.",
   TITLE="Multiple-breath washout is a marker of lung disease in preschool children with cystic fibrosis.",
   JOURNAL="Am. J. Respir. Crit. Care Med.",
   VOLUME="171",
   YEAR="2005",
   PAGES="249-256"
}

@ARTICLE{Monika2006,
   AUTHOR="Fuchs, S. I. and Buess, C. and Lum, S. and Kozlowska, W. and Stocks, J. and Gappa, M.",
   TITLE="Multiple breath washout with a sidesream ultrasonic flow sensor and mass spectrometry.",
   JOURNAL="Pediatric Pulmonology",
   VOLUME="41",
   YEAR="2006",
   PAGES="1218-1225"
}

%%Smoker
@ARTICLE{Sylvia_smoker,
   AUTHOR="Verbanck, S. and Schuermans, D. and Meysman, N. and Paiva, M. and Vincken, W.",
   TITLE="Noninvasive assessment of airway alterations in smokers: the small airways revisited.",
   JOURNAL="Am. J. Respir. Crit. Care Med.",
   VOLUME="170",
   YEAR="2004",
   PAGES="414-419"
}

%% LCI
@ARTICLE{Bouhuys1963,
   AUTHOR="Bouhuys, A.",
   TITLE="Pulmonary nitrogen clearance in relation to age in healthy males.",
   JOURNAL="J. Appl. Physiol.",
   VOLUME="18",
   YEAR="1963",
   PAGES="297-300"
}

@ARTICLE{Horsley2009,
   AUTHOR="Horsley, A. R.",
   TITLE="Lung clearance index in the assessment of airways disease.",
   JOURNAL="Respir. Med.",
   VOLUME="103",
   YEAR="2009",
   PAGES="793-799"
}

@ARTICLE{HorsleyCF,
   AUTHOR="Horsley, A. R. and Gustafsson, P. M. and Maceod, K. A. and Saunders, C. and Greening, A. P. and Porteous, D. J. and Davies, J. C. and Cunningham, S. and Alton, E. W. F. W. and Innes, J. A.",
   TITLE="Lung clearance index is a sensitive, repeatable and practical measure of airways disease with cystic fibrosis.",
   JOURNAL="Thorax",
   VOLUME="63",
   YEAR=2008"",
   PAGES="135-140"
}

@ARTICLE{LCI2008,
   AUTHOR="Davies, J. C. and Cunningham, S. and Alton, E. W. F. W. and Innes, J. A.",
   TITLE="Lung clearance index in CF: a sensitive marker of lung disease severity.",
   JOURNAL="Thorax",
   VOLUME="63",
   YEAR="2008",
   PAGES="96-97"
}
@ARTICLE{Kraemer2005,
   AUTHOR="Kraemer, R. and Blum, A. and Schibler, A. and Ammann, R. A. and Gallati, S.",
   TITLE="Ventilation inhomogeneity in relation to standard lung function in patients with cyctic fibrosis.",
   JOURNAL="Am. J. Respir. Crit. Care Med.",
   VOLUME="171",
   YEAR="2005",
   PAGES="371-378"
}

@ARTICLE{Kraemer2008,
   AUTHOR="Latzin, P. and Thamrin, C. and Kraemer, R.",
   TITLE="Ventilation inhomogeneities assessed by the multibreath washout (MBW) technique.",
   JOURNAL="Throax",
   VOLUME="63",
   YEAR="2008",
   PAGES="98-99"
}

@ARTICLE{Becklake1951,
   AUTHOR="Becklake, M. R.",
   TITLE="A new index of the intrapulmonary mixture of inspired air.",
   JOURNAL="Throax",
   VOLUME="7",
   YEAR="1952",
   PAGES="111-116"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{weibel_generation,
   AUTHOR="Weibel, E. R. and Sapoval, B. and Filoche, M.",
   TITLE="Design of peripheral airways for efficient gas exchange",
   JOURNAL="Respiratory Physiology and Neurobiology",
   VOLUME="148",
   PAGES="3-21",
   YEAR="2005"
} 

@ARTICLE{lung_SEM,
   AUTHOR="Weibel, E. R.",
   TITLE="{Fractal geometry: a design principle for living organisms}",
   JOURNAL="Am. J. Physiol. Lung Cell Mol. Physiol.",
   VOLUME="261",
   PAGES="L361-L369",
   YEAR="1991"
} 

@ARTICLE{Wiggs_airway_dimensions,
   AUTHOR="Wiggs, B. R. and Moreno, R. and Hogg, J. C. and Hilliam C. and Pare, P. D.",
   TITLE="{A model of the mechanics of airway narrowing}",
   JOURNAL="Journal of Applied Physiology",
   VOLUME="69",
   PAGES="849-860",
   YEAR="1990"
} 

@BOOK{Pulmonary_physiology,
  AUTHOR="Levitzky, M. G.",
  TITLE="Pulmonary Physiology",
  PUBLISHER = "McGraw-Hill" ,
  EDITION = "6th",
  YEAR = 2002,
}

%@ARTICLE{body_plethysmograph,
%   AUTHOR="DuBois, A. B. and Botelho, S. Y. and Comroe Jr., J. H. ",
%   TITLE="A new method for measuring airway resistance in man using body plethysmograph: values in normal subjects and in patients with respiratory disease",
%   JOURNAL="J. Clin. Invest.",
%   VOLUME="35",
%   PAGES="327-335",
%   YEAR="1956"
%} 


@BOOK{spirometry,
  AUTHOR="Johns, D. P. and Pierce, R.",
  TITLE="{Spirometry: the measurement and interpretatioon of ventilatory function in clinical practice}",
  PUBLISHER = "National Asthma Council, Melbourne" ,
  EDITION = "6th",
  YEAR = 2004,
}

@Article{wanger2005,
author = {Wanger, J. and Clausen, J. L. and Coates, A. and Pedersen, O. F. and Brusasco, V. and Burgos, F. and Casaburi, R. and Crapo, R. and Enright, P. and van der Grinten, C. P. M. and Gustafsson, P. and Hankinson, J. and Jensen, R. and Johnson, D. and MacIntyre, N. and McKay, R. and Miller, M. R. and Navajas, D. and Pellegrino, R. and Viegi, G.},
title = {{Standardisation of the measurement of lung volumes}},
journal = {Eur. Respir. J.},
volume = {26},
number = {3},
pages = {511-522},
year = {2005}
}

@BOOK{lung_function,
  AUTHOR="Cotes, J. E.",
  TITLE="{Lung Function: Chapter 15}",
  PUBLISHER = "Blackwell Scientific Publications" ,
  EDITION = "3rd",
  YEAR = 1975,
}

@article{MBNW_FRC,
author = {Wrigge, H. and Sydow, M. and Zinserling, J. and Neumann, P. and Hinz, J. and Burchardi, H.},
title={{Early Detection of Airways Obstruction by the Closing Volume Technique}},
journal = {Intensive Care Medicine},
volume = {24},
number = {5},
pages = {487-493},
year = {1998},
}

%%% Chapter 2 : MBNW and Gas Mixing %%%%%%%%%%

@ARTICLE{Baker1974,
   AUTHOR="Baker, L. G. and Ultman, J. S. and Rhodes, R. A.",
   TITLE="Simultaneous flow and diffusion in a symmetric airway system: a mathematical model.",
   JOURNAL="Respir. Physiol.",
   VOLUME="21",
   PAGES="119-138",
   YEAR="1974"
} 

@ARTICLE{Paiva_eq,
   AUTHOR="Paiva, M. and Paiva, V.",
   TITLE="Stochastic simulation of the gas diffusion in the air phase of the human lung.",
   JOURNAL="Bell. Math. Biophys.",
   VOLUME="34",
   PAGES="457-466",
   YEAR="1972"
} 

@BOOK{Chapman_Enskog,
   AUTHOR="Chapman, S. and Cowling, T. G.",
   TITLE="The Mathematical Theory of Nonuniform Gases.",
   PUBLISHER = "Cambridge University Press" ,
   EDITION = "3rd",
   YEAR = 1970,
}

@ARTICLE{Bohr1891,
   AUTHOR="Bohr, C.",
   TITLE="Ueber die Lungenatmung.",
   JOURNAL="Skand. Arch. Physiol.",
   VOLUME="2",
   PAGES="236-268",
   YEAR="1891"
} 

@ARTICLE{Fowler1948,
   AUTHOR="Fowler, W. S.",
   TITLE="Lung function studies. II. the respiratory dead space",
   JOURNAL="Am. J. Physiol.",
   VOLUME="154",
   PAGES="405-416",
   YEAR="1948"
} 

@ARTICLE{Kars1997,
   AUTHOR="Kars, A. H. and Bogaard, J. M. and Stijnen, T. and de Vries, J. and Verbaak, A. F. and Hilvering, C.",
   TITLE="Deadspace and slope indices from the expiratory carbon dioxide-tension volume curve.",
   JOURNAL="Eur. Respir. J.",
   VOLUME="10",
   PAGES="1829-1836",
   YEAR="1997"
} 

@ARTICLE{SBCO2,
   AUTHOR="Tusman, G. and Areta, M. and Climente, C. and Plit, R. and Suarez-Sipmann, F. and Rodr$\acute{i}$guez-Nieto, M. J. and Peces-arba, G. and Turchetto, E. and B$\ddot{o}$hm, S. H.",
   TITLE="Effect of pulmonary perfusion on the slopes of single-breath test of CO$_2$.",
   JOURNAL="J. Appl. Physiol.",
   VOLUME="99",
   PAGES="650-655",
   YEAR="2005"
} 

@ARTICLE{Piiper1976,
   AUTHOR="Sikand, R. S. and Magnussen, H. and Scheid, P. and Piiper, J. ",
   TITLE="Convective and diffusive gas mixing in human lungs: experiments and model analysis.",
   JOURNAL="J. Appl. Physiol.",
   VOLUME="40",
   PAGES="362-371",
   YEAR="1976"
} 




@ARTICLE{Lutchen1990,
   AUTHOR="Lutchen, K. R. and Habib, R. H. and Dorkin, H. L. and Wall, M. A.",
   TITLE="Respiratory impedence and multiplebreah N2 washout in healthy, asthmatic, and cystic fibrosis subjects.",
   JOURNAL="J. Appl. Physiol.",
   VOLUME="68",
   PAGES="2139-2149",
   YEAR="1990"
} 

@ARTICLE{Cumming1967,
   AUTHOR="Cumming, G.",
   TITLE="Gas mixing efficiency in the human lung.",
   JOURNAL="Respir. Physiol.",
   VOLUME="2",
   PAGES="213-224",
   YEAR="1967"
} 
@ARTICLE{Cutillo1972,
   AUTHOR="Cutillo, A. and Omboni, E. and Delgrossi, S.",
   TITLE="Effects of respiratory frequency on distribution of inspired gas in normal subjects and in patients with chronic obstructive lung disease.",
   JOURNAL="Am. Rev. Respir. Dis.",
   VOLUME="105",
   PAGES="756-767",
   YEAR="1972"
} 

@ARTICLE{Cutillo1981,
   AUTHOR="Cutillo, A. and Perondi, R. and Turiel, M. and Egger, J. and Watanabe, S. and Renzetti, A.",
   TITLE="Reprodusibility of multibreath nitrogen washout measurements.",
   JOURNAL="Am. Rev. Respir. Dis.",
   VOLUME="124",
   PAGES="505-507",
   YEAR="1981"
} 

@ARTICLE{Roos1955,
   AUTHOR="Roos, A. and Dahlstrom, H. and Murphy, J. P.",
   TITLE="Distribution of inspired air in the lungs.",
   JOURNAL="J. Appl. Physiol.",
   VOLUME="7",
   PAGES="645-659",
   YEAR="1954"
}


@ARTICLE{Crawford1985,
   AUTHOR="Crawford, A. B. H. and Makowska, M. and Paiva, M. and Engel, L. A.",
   TITLE="Convection- and diffusion-dependent ventilation maldistribution in normal subjects.",
   JOURNAL="J. Appl. Physiol.",
   VOLUME="59(3)",
   PAGES="838-846",
   YEAR="1985"
}






@article{phaseIV_mansell,
author = {Mansell, A. and Bryan, C. and Levison, H.},
title = {{Airway closure in children}},
journal = {J Appl Physiol},
volume = {33},
number = {6},
pages = {711-714},
year = {1972},
}

@article{phaseIV_SoniaBuist,
author = {Buist, A. Sonia},
title={{Early Detection of Airways Obstruction by the Closing Volume Technique}},
journal = {Chest},
volume = {64},
number = {4},
pages = {495-499},
year = {1973},
}

@article{Fowler1951,
author = {Fowler, W. S. and Cornish, E. R. and Seymour, S. K.},
title={{Lung Function Studies VIII. Analysis of Alveolar Ventilation by Pulmonary N2 Clearance Curves}},
journal = {J. Clin. Invest.},
volume = {31},
number = {1},
pages = {40-50},
year = {1952},
}

@article{Crawford1987,
author = {Crawford, A. B. H. and Makowska, M. and Engel, L A.},
title={{Effect of bronchomotor tone on static mechanical properties of lung and ventilation distribution}},
journal = {J. Appl. Physiol.},
volume = {62},
number = {6},
pages = {2278-2285},
year = {1987},
}

@ARTICLE{Paiva1979,
   AUTHOR="Paiva, M. and Engel, L. A.",
   TITLE="Pulmonary interdependence of gas transport.",
   JOURNAL="J. Appl. Physiol.",
   VOLUME="47",
   PAGES="296-305",
   YEAR="1979"
} 

@ARTICLE{Paiva1973,
   AUTHOR="Paiva, M.",
   TITLE="Gas transport in the humna Lung.",
   JOURNAL="J. Appl. Physiol.",
   VOLUME="35",
   PAGES="401-410",
   YEAR="1973"
} 

@ARTICLE{Sylvia1997,
   AUTHOR="Verbanck, S. and Schuermans, D. and Van Muylem, A. and Paiva, M. and Noppen, M. and Vicken, W.",
   TITLE="Ventilation distribution during histamine provocation.",
   JOURNAL="J. Appl. Physiol.",
   VOLUME="83",
   PAGES="1907-1916",
   YEAR="1997"
} 

@ARTICLE{Lewis1978e,
   AUTHOR="Lewis, S. M.",
   TITLE="Emptying patterns of the lung studied by multiple-breath N$_2$ washout.",
   JOURNAL="J. Appl. Physiol.",
   VOLUME="44",
   PAGES="424-430",
   YEAR="1978"
} 

@ARTICLE{Lewis1978c,
   AUTHOR="Lewis, S. M. and Evans, J. W. and Jalowayski, A. A.",
   TITLE="Continuous distributions of specific ventilation recovered from inert gas washout.",
   JOURNAL="J. Appl. Physiol.",
   VOLUME="44",
   PAGES="416-423",
   YEAR="1978"
}

@ARTICLE{Whiteley1999,
   AUTHOR="Whiteley, J. P. and Gavaghan, D. J. and Hahn, C. E. W.",
   TITLE="A tidal breathing model for the multiple inert gas elimination technique.",
   JOURNAL="J. Appl. Physiol.",
   VOLUME="87",
   PAGES="161-169",
   YEAR="1999"
}

@ARTICLE{Hahn1998,
   AUTHOR="Gavaghan, D. J. and Hahn, C. E. W.",
   TITLE="A tidal breathing model of the forced inspired inert gas sinewave technique.",
   JOURNAL="Respir. Physiol.",
   VOLUME="106",
   PAGES="209-221",
   YEAR="1996"
}
@ARTICLE{Farmery2000,
   AUTHOR="Farmery, A. D. and Hahn, C. E. w.",
   TITLE="Response-time enhancement of a clinical gas analyzer facilitates measurement of breath-by-breath gas exchange.",
   JOURNAL="J. Appl. Physiol.",
   VOLUME="89",
   PAGES="581-589",
   YEAR="2000"
} 

%%% Chapter 3 : MBHW System %%%%%%%%%%%%%%%%%%%
@article{Gluck1990,
author = {Gluck, E H and Onorato, D J and Castriotta, R},
title={{Helium-oxygen mixtures in intubated patients with status asthmaticus and respiratory acidosis.}},
journal = {Chest},
volume = {98},
number = {3},
pages = {693-698},
year = {1990}
}


@ARTICLE{TF_for_helium,
   AUTHOR="Blaauwgeers, R. and Blazkova, M. and $\check{C}$love$\check{c}$ko, M. and Eltsov, V. B. and Graaf, R. and Hosio, J. and Krusius, m. and Schmoranzer, D. and Schoepe, W. and Skrbek, L. and Skyba, P. and Solntsev, R. E. and Zmeev, D. E.",
   TITLE="Quartz Tuning Fork: Thermometer, Pressure- and Visometer for Helium Liquids",
   JOURNAL="J. Low Temp. Physics",
   VOLUME="146",
   PAGES="537-562",
   YEAR="2007"
} 

@ARTICLE{TF_AFM,
   AUTHOR="Giessibl, F. J.",
   TITLE="Atomic resolution on Si(111)-(7x7) by noncontact atomic force microscopy with a force sensor based on a quartz tuning fork",
   JOURNAL="Appl. Phys. Lett.",
   VOLUME="76",
   PAGES="1470-1472",
   YEAR="2000"
} 

@ARTICLE{TF_SF6,
   AUTHOR="Zeisel, D. and Menzi, H. and Ullrich, L.",
   TITLE="A precise and robust quartz sensor based on tuning fork technology for (SF$_6$)-gas density control",
   JOURNAL="Sensors and Actuators",
   VOLUME="80",
   PAGES="233-236",
   YEAR="2000"
} 

@ARTICLE{TF_liquid,
   AUTHOR="Zhang, J. and O'Shea, S.",
   TITLE="Tuning forks as micromechanical mass sensitive sensors for bio- or liquid detection",
   JOURNAL="Sensors and Actuators B",
   VOLUME="94",
   PAGES="65-72",
   YEAR="2003"
} 

@ARTICLE{Sader2006,
   AUTHOR="Van Eysden, C. A. and Sader, J. E.",
   TITLE="Resonant Frequencies of a Rectangular Cantilever Beam Immersed in a Fluid",
   JOURNAL="J. Appl. Physics",
   VOLUME="100",
   PAGES="114916",
   YEAR="2006"
} 

@ARTICLE{Cleveland_TF,
   AUTHOR="Cleveland, J. P. and Manne, S. and Bocek, D. and Hansma, P.K.",
   TITLE="A nondestructive method for determining the spring constant of cantilevers for scanning force microscopy",
   JOURNAL="Rev. Sci. Instrum.",
   VOLUME="64(2)",
   PAGES="403",
   YEAR="1993"
}

@ARTICLE{Chu_TF,
   AUTHOR="Chu, W. H.",
   TITLE="DTMB Contract Nobs-86396",
   JOURNAL="Southwest Research Institute Technical Report No. 2",
   VOLUME="X",
   PAGES="NObs86396",
   YEAR="1963 (unpublished)"
} 

@ARTICLE{beam_vib,
   AUTHOR="Han, S. M. and Benaroya, H. and Wei, T.",
   TITLE="Dynamics of transversely vibrating beams using four engineering theories",
   JOURNAL="Journal of Sound and Vibration",
   VOLUME="225",
   PAGES="935-988",
   YEAR="1999"
}
 
@ARTICLE{Sader1998,
   AUTHOR="Sader, J. E.",
   TITLE="Frequency response of cantilever beams immersed in viscous fluids with application to the atomic microscope",
   JOURNAL="J. Appl. Physics",
   VOLUME="84",
   NUMBER="1",
   YEAR="1998"
} 

@BOOK{Smith,
  AUTHOR="Sedra, A. S. and Smith, K. C.",
  TITLE="Microelectronic Circuits",
  PUBLISHER = "Oxford University Press" ,
  EDITION = "5th",
  YEAR = 2004,
}

@ARTICLE{AFM_saitoh,
   AUTHOR="Saitoh, K. and , Hayashi, K. and Shibayama, Y. and Shirahama, K.",
   TITLE="A low temperature scanning probe microscope using a quartz tuning fork",
   JOURNAL="J. Physics: Conference Series",
   VOLUME="150",
   NUMBER="012039",
   YEAR="2009"
} 

@ARTICLE{AFM_yoshiaki,
   AUTHOR="Yoshiaki Sugimoto and Seiji Innami and Masayuki Abe and Oscar Custance and Seizo Morita.",
   TITLE="Dynamic force spectroscopy using cantilever higher flexural modes",
   JOURNAL="Appl. Phys. Lett.",
   VOLUME="91",
   NUMBER="9",
   PAGES="093120",
   YEAR="2007"
} 

@ARTICLE{AFM_hasegawa,
   AUTHOR="Hasegawa, Y. and Eguchi, T.",
   TITLE="Potential profile around step edges of Si surface measured by nc-AFM",
   JOURNAL="Appl. Surf. Sci.",
   VOLUME="188",
   NUMBER="3-4",
   PAGES="386-390",
   YEAR="2002"
} 

@ARTICLE{AFM_pinto,
   AUTHOR="Pinto, H. P. and Enevoldsen, G. H. and Besenbacher, F. and Lauritsen, J. V. and Foster, A. S.",
   TITLE="The role of tip size and orientation tip-surface relaxations and surface impuries in simultaneous AFM and STM",
   JOURNAL="Nanotechnology",
   VOLUME="20",
   NUMBER="9pp",
   PAGES="264020",
   YEAR="2009"
}
 
@ARTICLE{AFM_kunstmann,
   AUTHOR="Kunstmann, T. and Fendrich, M. and Paulkowski, D. and Wagner, Th. and M$\ddot{o}$ller, R.",
   TITLE="Combined normal and torsional mode in frequency-modulation atomic force microscopy for lateral dissipation measurement",
   JOURNAL="Appl. Phys. Lett.",
   VOLUME="88",
   NUMBER="15",
   PAGES="153112",
   YEAR="2006"
} 

@ARTICLE{Infrared_abs,
   AUTHOR="Nielsen, J. R. and Thornton, V. and Dale, E. B.",
   TITLE="The Absorption Laws for Gases in the Infra-red",
   JOURNAL="Rev. Mod. Physics",
   VOLUME="16(3)",
   PAGES="307",
   YEAR="1944"
} 

@ARTICLE{IR_CO2,
   AUTHOR="Martin, P. E. and Barker, E. F.",
   TITLE="The Infrared Absorption Spectrum of Carbon Dioxide",
   JOURNAL="Phys. Rev.",
   VOLUME="41",
   PAGES="291-303",
   YEAR="1932"
} 

@BOOK{Bube,
  AUTHOR="Bube, R. H.",
  TITLE="Photoconductivity of solids",
  PUBLISHER = "Wiley" ,
  EDITION = "1st",
  YEAR = 1960,
}


@ARTICLE{photoconductivity,
   AUTHOR="Wright, D. A.",
   TITLE="Photoconductivity",
   JOURNAL="British J. Appl. Phys.",
   VOLUME="9",
   PAGES="205",
   YEAR="1958"
} 

@ARTICLE{Humphery1957,
   AUTHOR="Humphery, J. N.",
   TITLE="Photoconductivity in Lead Selenide. Experimental.",
   JOURNAL="Phys. Rev.",
   VOLUME="105",
   PAGES="469",
   NUMBER="2",
   YEAR="1957"
} 

@ARTICLE{Humphery1957Theo,
   AUTHOR="Humphery, J. N.",
   TITLE="Photoconductivity in Lead Selenide. Theory of the Mechanism of Sensitization.",
   JOURNAL="Phys. Rev.",
   VOLUME="105",
   PAGES="1736",
   NUMBER="6",
   YEAR="1957"
} 

@Article{Humphery1957Sen,
  title = {Photoconductivity in Lead Selenide: Theory of the Dependence of Sensitivity on Film Thickness and Absorption Coefficients},
  author = {Humphrey, James N. and Petritz, Richard L.},
  journal = {Phys. Rev.},
  volume = {105},
  number = {4},
  pages = {1192--1197},
  numpages = {5},
  year = {1957},
}

@ARTICLE{petritz1956,
   AUTHOR="Petritz, R. L.",
   TITLE="Theory of Photoconductivity in Semiconductor films",
   JOURNAL="Phys. Rev.",
   VOLUME="104",
   PAGES="1508-1516",
   YEAR="1956"
} 

@Article{harada1956,
  title = {Photosensitization of PbS Films},
  author = {Harada, R. H. and Minden, H. T.},
  journal = {Phys. Rev.},
  volume = {102},
  number = {5},
  pages = {1258--1262},
  numpages = {4},
  year = {1956}
}

@Article{US6218665,
  title = {Infrared detector and gas analyzer},
  author = {Yamamori, S. and Dainobu, H.},
  journal = {US Patents},
  number = {6218665},
  year = {2001}
}

@Article{US4578762,
  title = {Self-calibrating carbon dioxide analyzer},
  author = {Wong, J. Y.},
  journal = {US Patents},
  number = {4578762},
  year = {1986}
}

@ARTICLE{1N4007diode,
   AUTHOR="Nanda, K. K. and Sarangi, S. N.",
   TITLE="Electrical Properties of 1N4007 Silicon Diode.",
   JOURNAL="Rev. Sci. Instrum.",
   VOLUME="68",
   PAGES="2904",
   NUMBER="7",
   YEAR="1997"
} 

@BOOK{fluid_dynamics,
  AUTHOR="Batchelor, G. K. ",
  TITLE="{An Introduction to Fluid Dynamics}",
  PUBLISHER = "Cambridge University Press" ,
  EDITION = "2nd ",
  YEAR = 2006,
}

@ARTICLE{Smith_piezoresistance,
   AUTHOR="Smith, C. S.",
   TITLE="Piezoresistance Effect in Germanium and Silicon.",
   JOURNAL="Phys. Rev.",
   VOLUME="94",
   PAGES="42",
   NUMBER="1",
   YEAR="1954"
} 

@ARTICLE{Herring_piezoresistance,
   AUTHOR="Herring, C and Vogt, E.",
   TITLE="Transport and Defromation-Potential Theory for Many-Valley Semiconductors with Anisotropic Scattering.",
   JOURNAL="Phys. Rev.",
   VOLUME="101",
   PAGES="944",
   NUMBER="3",
   YEAR="1956"
} 

@ARTICLE{Long_silicon_diaphragm,
   AUTHOR="Tufte, O. N. and Chapman, P. W. and Long, D.",
   TITLE="Silicon Diffused-element Piezoresistive Diaphragms.",
   JOURNAL="J. Appl. Physics",
   VOLUME="33",
   PAGES="3322",
   NUMBER="11",
   YEAR="1962"
} 

@ARTICLE{viscosity_air,
   AUTHOR="Lemmon, E. W. and Jacobsen, R. T.",
   TITLE="Viscosity and Thermal Conductivity Equation for Nitrogen, Oxygen, Argon, and Air.",
   JOURNAL="Int. J. Thermophys.",
   VOLUME="25",
   PAGES="21-65",
   NUMBER="1",
   YEAR="2004"
} 

@BOOK{Photoconductor_art,
  AUTHOR="Joshi, N. V.",
  TITLE="Photoconductivity: Art, Science and Technology (Optical Engineering)",
  PUBLISHER = "CRC Press" ,
  EDITION = "1st",
  YEAR = 1990,
}


%%%%%%Chap 5 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%


